Estimating the Impact of Unknown Unknowns on Aggregate Query Results

It is common practice for data scientists to acquire and integrate disparate data sources to achieve higher quality results. But even with a perfectly cleaned and merged data set, two fundamental questions remain: (1) is the integrated data set complete and (2) what is the impact of any unknown (i.e., unobserved) data on query results? In this work, we develop and analyze techniques to estimate the impact of the unknown data (a.k.a., unknown unknowns) on simple aggregate queries. The key idea is that the overlap between different data sources enables us to estimate the number and values of the missing data items. Our main techniques are parameter-free and do not assume prior knowledge about the distribution. Through a series of experiments, we show that estimating the impact of unknown unknowns is invaluable to better assess the results of aggregate queries over integrated data sources.

==> cover_letter.tex <==

\section*{Dear SIGMOD Group Leader and Referees:}
We thank the reviewers and group leader for the very helpful feedback on our paper. We have addressed all of the listed concerns and include references to the revised text in the cover letter. To summarize :


\begin{itemize}
\item We added an extensive example with illustrations to the appendix. We show by means of a toy example how the f-statistic and the {\em \naive}, {\em frequency} and {\em bucket} estimators are calculated. We further sketch how the estimation quality improves if we add an additional data source. 
\item We added a summary section to the evaluation section to summarize the insights/lessons learned, and provided a theoretical discussion about the usefulness of the estimators in practice. 
\item We added additional experiments to the appendix for completeness. 
\item We improved the presentation of Sections 3.1, 3.3. and 3.4.
\end{itemize}

\section*{Meta Reviews}
{\bf M1.} {\em The authors are requested to address their requests for clarification, in particular, technical details in sections 3.1, 3.3 and 3.4 need to be clarified and illustrated. }

{\bf Responses:} We took Reviewer 1's  comment by heart and included an illustrated example (Appendix~\ref{appendix:toy}) that shows how the various estimators perform on the same abstracted example. 
Unfortunately, as with almost all statistics very small examples are hard to convey any statistical properties, which makes any calculation by hand hard to follow. 
Therefore, our only option was to derive a very small data set, which can demonstrate how the different estimators work and why one is better than another for that particular example. 
We added the example to the appendix due to space constraints and to avoid interrupting the reading flow.
Especially, we do not want to confuse the reader with the fact, that slight modifications of the example could yield completely different outcomes as to which estimator is better or worse; something that is only possible because of the small size of the example.
Finally, we wanted to align the paper in style more to other papers in the space (e.g., the VLDB paper by Peter Haas \cite{haas}, which uses species estimation to determine the number of distinct values within a database table of known size), and usually also do not have toy examples in the main text.
However, if the reviewers feel strongly about it, we will incorporate the example into the main text for the camera ready-version. 
\\


{\bf M2.} {\em The authors are also asked to provide a summary of insights/lessons learned and experiments or theory assessing the usefulness of the estimates.}


{\bf Responses:} We added a new subsection, Section~\ref{sec:eval:summary}, which discusses the lessons learned and the usefulness of the estimates in practice. 
In this subsection, we summarize the findings and give suggestions regarding which estimator to use. 
Furthermore, we discuss how much trust the user can put into the estimates based on our findings and the vast amount of experience statisticians have with species estimation techniques. 
However, as Reviewer 2 also pointed out, this work can be best regarded as a first step into a new field and we cannot answer all the questions in one paper. Rather, we believe that this work might open up a new line of research.

\section*{Reviewer 1}
{\bf A1.} {\em "For the purpose of this work, we assume that data sources are independent" My understanding of the paper is that the publicity score compensates for this otherwise limiting assumption. Maybe you want to explain that early.}

{\bf Responses:} With independence we meant that the data sources are independent samples and not copies of each other. If they would be copies, we have effectively only one data source and no statistical inference would be possible. We therefore changed the sentence to: "For the purpose of this work, we assume that data sources are independent samples (e.g., data sources are not copies from each other and instead are independently created)". 
That does not mean, that different data sources cannot include the same companies. On the contrary, as you pointed out, by means of the publicity score this will exactly be the case. 
\\

{\bf A2:} {\em I have difficulties following the discussion right after equation 9. The text is well written, but assumes a lot of familiarity with various concepts that could be simply understood with the help of an abstracted running example (with concrete numbers and a few figures). Can you please include an illustrating example (perhaps with some assumed value distributions inspired by real data you found) that shows how these various estimators perform on the same abstracted example, and that give more intuition of why 3 better 2 better 1.}

{\bf Responses:} Thanks for this valuable comment. We followed your suggestion as explained above. 
\\

{\bf A3:} {\em  Bucket estimator: for your company example. Don't we have: more employees -> more publicity? Your bucket estimator seems to ignore this overall correlation. E.g., it would be a priori possible that the order of publicity value in decreasing order is: small, large, medium enterprises. Wouldn't an a priori assumption of large, medium, small (thus some correlation based on the actual values) work better? }

{\bf Responses:} Great point. This is exactly what the dynamic bucket estimator does and the reason why it works better. However, it does so without requiring a specific a priori assumption set by the user. The bucket estimator reduces the number of buckets if and only if it reduces the estimated value (see Section~\ref{sum:bucket:dynamic}). 
Let us consider a simple toy example consisting of 50 small companies with 10 employees each and 50 big companies with 10000 employees. Let us further assume that the small companies have a lower publicity likelihood and all the big companies have been observed but 10 small companies are still missing. 
Finally, let us assume that the unknown count estimate (e.g., Chao91) is exactly 10 missing companies.
Hence, the  \naive estimator would estimate a total sum of $50*1000 + 40 * 100 + 10 * (50*10000 + 40*100) / 90 = 560000$ employees. That is the sum over all observed companies ($50*1000 + 40 * 100$), plus the number of unobserved companies ($10$) times the average value of the observed companies ( $ 10 * (50*10000 + 40*100) / 90 $). 

The bucket estimator on the other hand will split the value range into two: a high range bucket and a low range bucket. 
It will not try to split the range further as we designed the example in a way that all missing companies have the exact same number of employees. 
Thus, the estimator will find that in the high-range bucket, the one containing the big companies, no missing values exists, whereas it would estimate missing companies for the small-range bucket. 
Thus, the final estimate is $50*1000 + 40 * 100 + 10 * ( 40*100) / 40 = 505000$. The sum over all observed companies ($50*1000 + 40 * 100$) plus  the number of unobserved companies ($10$) times the average value of the observed companies in the small bucket range ( $ 10 * ( 40*100) / 40 $). 
In this case, the overall estimate would is $505000$ - a much better estimate, which is in this case equivalent to the ground truth.  

The appendix now contains a more detailed and concrete toy example and illustration. 
\\

{\bf A4:} {\em "Second, the values per bucket are more similar, making the estimate less sensitive to extreme values (proof is trivial and omitted)." First, please include the proof in the appendix. Second, smaller bucket size, means fewer data points, means less accurate estimation. It is not clear from a first glance that reducing "extreme values" more than compensates for less accurate estimation per bucket (or perhaps I am just missing something super trivial. Please elaborate) }

{\bf Responses:} We indeed meant something trivial by it. Let us assume the value range (e.g., the number of employees in the consolidated database) ranges from 1 to 100. 
Thus, the difference between the largest and smallest value in the range is 99.
If we now split the bucket into two, e.g., from 1 to 50 and 51 to 100, the maximum difference is 49. 
Thus, the values per bucket are much more {\em similar}. 
Now assume that we have a lot of companies in the range from 1 to 100, but one single company with a value of 10000. 
If we calculate the average over all companies, this one single outlier has a profound effect. 
However, if we split the companies again from 1 to 50 and 51 to now 10000, only the last bucket is impacted by the really high value and the total estimate is more robust as only the buckets at the boundary of the value range might be impacted.

However, it is also true that if the buckets are too small, the estimation accuracy suffers. Something our dynamic bucket strategy carefully considers (see Section~\ref{sum:bucket:dynamic}).

In the paper, we carefully reworded the paragraph to make this clearer. 



{\bf A5:} {\em Static estimator: why would you bucket by equally partitioning the values instead of making the buckets of equal size? The later seems a straight-forward more intuitive naive implementation, justified by the need to provide enough samples for each bucket? }

{\bf Responses:} Thank you, that is a very good point. In fact, we already did experiments with both static bucket approaches: the equi-width approach described in the paper and the equi-height approach you suggested (i.e., divide the observed sample, sorted by value, evenly into a fixed number of buckets). 
We only included one of them, as the dynamic approach always dominates the static approaches. 
The problem with all static bucket estimates is that it is impossible to determine the optimal number or size of buckets without knowing the ground truth.
For completeness, we added Appendix~\ref{appendix:static} to compare how different types and variations of the equi-height and equi-width static bucket estimators perform between each other as well as compared to the dynamic and naive methods. 
\\

{\bf A6:} {\em  Sec 3.4.: Here I have difficulties following the overall motivation: how does MC simulations help you estimate the underlying distributions better? And what do the parameter $\theta$ and $Q_\theta$ stand for? }

{\bf Responses:} A major drawback of sample-coverage based (unknown count) estimation (e.g., $Chao92$) is that it requires a single sample \em{WITH} replacement from the underlying truth. 
This is usually not a problem, if enough data sources exist and every data source contributes more or less the same number of data items (recall, that data sources are assumed to sample for the ground truth \em{WITHOUT} replacement); in this case, the integrated data set is similar enough to a single sample \em{WITH} replacement. 
However, if one data source contains a lot more information than another, this can be problematic as it is no longer a ``good'' sample \em{WITH} replacement. 
In this particular case, the {\em Monte-Carlo} method helps as it is not a frequentist method, and ignores how much data a specific data source contributes.
Instead, by means of {\em Monte-Carlo} simulation we try the best number of unknown items, which explains the number of observed data items per individual data source. 
This makes the estimator much more robust for uneven contributions from data sources (i.e., {\em streakers}) and a low number of data sources, but comes with its own limitations as discussed in Section~\ref{sec:eval:employee}.

In the paper, we improved the motivation of the MC method and now give the intuition behind it early on. 
\\

{\bf A7:} {\em  The experiments are very thorough, well thought through and carried out. Minor comment: The vertical axis in some of the plots starts at high numbers (e.g., 80 out of 480). What happens between 0 and 80? It's ok to show those ranges even if it has worse estimates (as in Fig 5b) }

{\bf Responses:} We unified all x-axis so that they start with 30. We do not show anything before 30 as it is a well-known rule-of-thumb  in statistics (even though a controversial one) that with less than 30 data points almost no estimations are possible. 
\\

\section*{Reviewer 2}
Thank you so much for the very kind review. We were happy to read that you liked it that much. 

\section*{Reviewer 3}
{\bf C1:} {\em  For the paper to be useful in practice, one would want to see some clear-cut lessons learned on when to apply which estimator, and (more) tight bounds that reflect the absolute (or relative) accuracy of the estimates, given the number of samples seen so far.}

{\bf Responses:} We added an entire new subsection to address this concern (Section~\ref{sec:eval:summary}). We also added additional experiments regarding the sample coverage (i.e., sample seen so far compared to the assumed population size) to backup the recommendations (Appendix~\ref{appendix:num_sources}).
\\

{\bf C2:} {\em  Taking the observed data only as an estimator performs quite good for the real world data.}

{\bf Responses:} Obviously, the observed data should at some point be the same as the estimate, otherwise they will not converge.
That said, the estimators clearly provide the biggest advantage the least complete the data set is. 
For example, in Figure~\ref{fig:real_employee} after 500 answers the number of observed items never approaches even the ``real'' number of employees in our experiment, whereas our bucket estimator is only off by a few percent.  
In contrast, for the revenue case (Figure~\ref{fig:real_source}(a)) with 500 answers both the number of observed data points and the estimation are equally good. 
However, if the collected data set is less complete (e.g., contains less than 300 crowd-answers), the bucket estimator is always much closer to the ground truth. 
Thus, the benefit of the estimates clearly depend on the ``completeness'' of the result. 
Even better, the estimators can be used to estimate how complete the result is; the closer the estimate to the observed value, the more complete the result (this is what the sample coverage estimate does). 
\\

{\bf C3:} {\em At times, in Section 3, equations and assumptions were not sufficiently motivated or alternatives not evaluated. }

{\bf Responses:} We generally improved the presentation of Section 3 and spent quite a bit of time on Section~\ref{sec:sum:mc} to better motivate the {\em Monte Carlo} estimator. Furthermore, we have included a couple of sections in Appendices to present evaluation results of other alternatives (Appendix~\ref{appendix:static} and \ref{appendix:other_estimators}) and also explain why we do not consider these alternatives in the paper. 
\\

{\bf C4:} {\em  It is written in the experimental evaluation section that other techniques are omitted, as ..... I suppose that means that these alternatives performed consistently (always) worse than Naive or Freq.}

{\bf Responses:} Often, they performed very similar to the ones we present in this paper, thus not justifying the complexity, and making the figures very hard to read. Instead of leaving them out entirely, we now decided to include them in Appendix~\ref{appendix:other_estimators} for completeness with more detailed explanations.
\\

{\bf C4:} {\em The paper is overall well written and organized, it was a good read.}

{\bf Responses: Thanks!} 
\\


\newpage


==> sum_query.tex <==
\vspace*{-10pt}
\section{Sum Query} \label{sec:sum}
Estimating the impact of unknown on aggregate sum query results is equivalent to solving two sub-problems: one is unknown data item count estimation, and the other is unknown data item value estimation. 
This directly relates to Definition~\ref{def:unknown_impact} and we focus on aggregate sum query to illustrate the proposed techniques.Such techniques can easily be extended to other queries such as count, average; in Section~\ref{sec:other_query}, we discuss how we can leverage the impact of unknown to drive count, avg and min/max queries.

The estimated impact of unknown, $\phi_{adj}$, can be used to adjust the original query result, $\phi_{obs}$, based on only observed data items.
\label{subsec:naive}
\begin{equation}\label{eqn:naive}
\phi_{sum} = \phi_{obs} + \phi_{adj}
\end{equation}

\subsection{Na{\"i}ve Estimator}
\label{sec:sum:naive}
As a Na{\"i}ve estimator, we use $Chao92$, which is derived under the open-world assumption, to estimate the number of unknown missing data items and assign the average value over the observed data items to the unknown data items. 
\begin{equation}\label{eqn:adj_chao}
\phi_{adj} = \frac{\phi_{obs}}{c}\cdot (\hat{N}_{Chao92}-c)
\end{equation}

Sampling-based estimation is inevitable under the open-world assumption, and the choice of a better sampling-based count estimator is difficult due to the fact that all the sampling-based estimators are sensitive to data skew \cite{haas}. We use $Chao92$ for unknown count estimation because it incorporates data skew in its estimation. 

We na{\"i}vely assign the average of observed distinct values to the unknown data items; however, this becomes very inaccurate if the sample is biased, as illustrated in Figure~\ref{fig:sample_bias}.

Alternatively, we can estimate the unknown values based on the singletons instead of all observed unique items (i.e., distinct values). Singletons, $f1$ are the data items that appears only once in the sample. Singletons are the most rare items in the sample, and if singletons are the best indicator of the missing data items, and then the values of the missing data items may be better represented by the average over the singletons, $\sfrac{\phi_{f_1}}{|f_1|}$.
\begin{equation}\label{eqn:adj_f1}
\phi_{adj} = \frac{\phi_{f_1}}{|f_1|}\cdot (\hat{N}_{Chao92}-c)
\end{equation}

\subsection{Bucket Estimator}
\label{subsec:bucket}
It is shown that no single estimator is optimal for all distributions with varying degrees of data skew, and even $Chao92$ is sensitive to the skewness in data [Haas, Naughton, Sehadri and Stokes]. Here, we propose an algorithm to compensate the $Chao92$ based Na{\"i}ve estimator to work with all distributions with varying degrees of data skew. In simple, we divide the observed value range for observed data items (i.e., bucket) into smaller sub-buckets and apply the Na{\"i}ve estimator at a finer-granularity.
\begin{equation}\label{eqn:bucket}
\phi_{bucket} = \sum_{b_i}{\phi_{b_i}}
\end{equation}
\subsubsection{Static bucket}
A static bucket is defined as a set with fixed boundaries: $b_i = \{x \in \mathbb{R} | x_{min} + w_i \cdot (i-1) \leq x < x_{min} + w_i \cdot i\}$. The width of each bucket, $w_i$, is equivalent for all $i$ and defined as follows:
\begin{equation}\label{eqn:bucket_static}
w_i = \frac{(x_{max}-x_{min})}{n_{b}}
\end{equation}

The optimal number of buckets varies depending on the underlying distribution. In general, having too few buckets will suffer from data skew (for count estimation) or even sample bias (for value estimation), whereas having too many buckets would leave each bucket with insufficient data to perform any estimations.

\subsubsection{Dynamic bucket}
The number of buckets for a better estimation may vary depending on the underlying distributions (i.e., varying degrees of data skew), and, worse yet, the underlying distributions are not known in advance; hence, we cannot guess-and-check different sets of buckets to fit the data. For the bucket estimator to work in practice, buckets need to be dynamically defined. In specific, we split a bucket into smaller ones to reduce data skew as well as sample bias.

Bucket splitting leaves us with a couple of questions to be addressed: when to split a bucket (i.e., splitting condition) and how to split (i.e., sub-bucket sizes). Furthermore, our goal is to compensate the $Chao92$ based Na{\"i}ve estimator without knowing the underlying distributions; this requires a parameter-free bucket splitting scheme that works with any distributions. Algorithm~\ref{alg:dynamic_bkt} describes the proposed {\em{Dynamic Bucket}} algorithm.

\begin{algorithm}[H]\label{alg:dynamic_bkt}
\IncMargin{1em}
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Indm
\Input{a bucket $b_0$ with a sample of size $n$}
\Output{an array of buckets of size $n_b$}
\Indp
\BlankLine
    $bkts = []$\tcc*[r]{an empty array}
    $n_b = bkts.size$\tcc*[r]{$n_b=0$}
    $bkts.add([b_0]$)\;
    \BlankLine
    \While{$n_b < bkts.size$}{
        $n_b = bkts.size$\;
        \For{$b \in bkts$}{
            $S_b = b.sample$\tcc*[r]{sample within $b$}
            $c_b = uniq(S_b)$\tcc*[r]{numb of unique items}
            $\hat{\gamma} = cv(S_b)$\tcc*[r]{coeff of variance}
            \BlankLine
            \If(\tcc*[f]{$^1c1$}){$c_b > 3 \land \hat{\gamma} \geq 0.05$}{
                $x_s = \underset{x \in S_b}
                {\arg\min}\{\underset{b_i\in split(b,x)}{\sum sum(b_i)}\}$\tcc*[r]{$^2c2$}
                $bkts.add([split(b,x_s)])$\;
            }
        }
    }
    \BlankLine
    return $bckts$\;
    \caption{Dynamic bucket generation}
\end{algorithm}
\DecMargin{1em}

The basic idea of the algorithm is to start from a single bucket, $b_0=\{x \in \mathbb{R} | x_{min} \leq x \leq x_{max}\}$ that contains the entire sample, and then iteratively split the bucket until the splitting condition no longer holds in any of the sub-buckets$^{c1}$. The splitting condition is based on the relationship between number of examples $n$, data skew $\gamma$ and margin of error $e$ for estimates in estimating the population mean \cite{n_e_cv}, which is our unknown value estimator for buckets:
\begin{equation}\label{eqn:lynch_kim}
n = \frac{z^2 \cdot \gamma^2}{e^2}
\end{equation}
For instance, at least 3 data items with $\gamma \leq 0.05$ are needed to estimate the unknown statistic, $\phi$, within $5\%$ margin of error at $95\%$ confidence (i.e., $z=1.96$). Using this as a guideline, $^1$we split only if the bucket has more than 3 unique data items with $\hat{\gamma} \leq 0.05$. Note that, since we approximate $\gamma$ with $\hat{\gamma}$, we condition on having at least 3 data classes, which is more strict than conditioning on 3 data items. In this way, all buckets would have a sufficient number of data items to estimate the mean (i.e., unknown value estimator for the bucket) within $5\%$ margin of error at $95\%$ confidence; furthermore, smaller buckets would contain relatively more uniform data (i.e., similar values), which reduces data skew for $Chao92$-based estimation. There is no tight bounds on $Chao92$ estimation (i.e., unknown count estimation for the bucket) to guide us in bucket generation, but we will investigate this further in the near future. 

The splitting condition can be easily adjusted using equation~\ref{eqn:lynch_kim} for different levels of margin of error. When a bucket meets the splitting condition, it splits into two sub-buckets on the most underestimating point$^{c2}$, which yields the smallest sum of the estimations on the sub-buckets. \yeounoh{Why underestimating is favored?}

\yeounoh{possibly come up with accuracy bounds - maybe lower bound}

\subsection{Monte-Carlo Estimator}
\label{subsec:mc}
The $Chao92$ species estimation technique assumes sampling with replacement and, thus, the proposed (Na{\"i}ve and Bucket) estimators require a sample with sufficient overlaps or duplicates. In this work, we assume that each source provides unique pieces of information without duplicates (i.e., sampling without replacement) as data vendors should do so in the real world, and the only way to observe more overlaps within the merged sample is to identify more independent sources.  We now turn to a Monte-Carlo estimator to compensate for the sampling of $Chao92$ and work directly with the per source samples without duplicates.

\subsubsection{Monte-Carlo method}
We know the sampling assumption (i.e. sampling without replacement), the number of sources as well as the number of examples per source. Can we model the true sampling distribution directly from these pieces of information and estimate the aggregation query result? We can formulate this into an optimization problem as follows:
\begin{equation}\label{eqn:mc_problem}
\min_{\theta}D_{KL}(P_{S}||Q_{\theta})
\end{equation}
\begin{comment}
=\min_{\theta}\sum_x{p_{S}(x)\cdot\ln\frac{q_{\theta}(x)}{p_{S}(x)}
\end{comment}
Kullback-Leibler (KL-) divergence, $D_{KL}$, measures the difference between two probability distributions, namely the observed sample distribution $P_{S}$ and a simulated sample distribution $Q_{\theta}$. KL-divergence is convex and non-negative \cite{lexa2004useful}, and we want to find the optimal parameter, $\theta=<\hat{N}>$, that will minimize the cost function (i.e., KL-divergence) given $P_{S}$ and $Q_{\theta}$, which is then simulated under the prescribed constraints: sampling without replacement, a fixed number of sources and the number of examples per source. To solve this optimization problem, we use Monte-Carlo method in conjunction with the Na{\"i}ve estimator. 

\begin{algorithm}\label{alg:mc_method}
\IncMargin{1em}
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Indm
\Input{an array of samples, $S_w$, with a sample from each source, $w_i$\\
        the number of unique data items, $\hat{N}$\\
        the number of simulations, $n_r$}
\Output{average KL-divergence value for the simulations}
\Indp
\BlankLine
    $n_w = S_w.size$\tcc*[r]{number of sources}
    $U = dist(\hat{N})$\tcc*[r]{sample dist for $\hat{N}$ items}
    $D_{KL} = 0.0$\tcc*[r]{default value}
    \BlankLine
    \For{$r = 1$ \KwTo $n_r$}{
        $Q_w = []$\tcc*[r]{simulated model}
        \For{$i = 1$ \KwTo $n_w$}{
            $s_i=sample(U,S_w[i].size)$\tcc*[r]{w/o repl}
            $Q_w.add([s_i])$
        }
        $S'_w,Q'_w=smooth(S_w,Q_w)$\tcc*[r]{$^3$smoothing}
        $D_{KL}\mathrel{+}=klDiv(S'_w,Q'_w)$\tcc*[r]{KL-divergence}
    }
    \BlankLine
    return $D_{KL}/n_r$\;
    \caption{Monte Carlo method for $D_{KL}(P_{S}||Q_{\theta})$}
\end{algorithm}
\DecMargin{1em}

The Monte Carlo method described in algorithm~\ref{alg:mc_method} allows us to compute the desired KL-divergence between observed and simulated sample distributions with a varying $\theta$; we select $\theta$ with the minimum KL-divergence and use it for the Na{\"i}ve estimator (equation~\ref{eqn:adj_chao} or \ref{eqn:adj_f1}). Although the KL-divergence cost function is convex, the integer parameter variable  $\hat{N}$ prevents us from using tractable optimization algorithms (e.g., gradient descent). Instead, we use $Chao92$ estimator to limit our parameter search space to $\{\theta \in \mathbb{N} | (1-\alpha)\cdot \hat{N}_{Chao92} \leq \theta \leq (1+\alpha)\cdot \hat{N}_{Chao92}\}$. 

We assume a uniform distribution for the underlying sample distribution of $Q_{\theta}$, and each source, $w_i$, samples $|w_i|$ examples without replacement. Other distributions that model skewed sample and publicity-value correlation can be used instead by introducing another variables in $\theta$; however, because the Na{\"i}ve estimator requires only the number of unique data items, we gain very little by modeling the sample skew. In addition, the observed sample may not contain $\hat{N}$ unique data items, in which case KL-divergence is not defined; we use smoothing$^3$ to assign a small non-zero probability to the missing extra unique items.

\subsubsection{Item Indexing}
KL-divergence, $D_{KL}(P_{S}||Q_{\theta})$, measures the information lost when $Q_{\theta}$ is used to approximate $P_{S}$; and the function is well-defined for both continuous and discrete distributions:
\begin{equation}\label{eqn:kl_disc}
D_{KL}(P_{S}||Q_{\theta})=\sum_{i}P_{S}(i)\cdot\ln{\frac{P_{S}(i)}{Q_{\theta}(i)}}
\end{equation}
To compute $D_{KL}(P_{S}||Q_{\theta})$, we only consider the discrete case in equation~\ref{eqn:kl_disc} for the following reasons. The number of unique data items, $\hat{N}$, is countably infinite (i.e., enumerable), and the real values for unknown data items are unknown. So rather than having a certain publicity for every possible attribute value, each item is assigned an index $i$ that indicates the ranking of its attribute value (e.g., index 2 indicates that the item has the second largest value within the sample) and the associated publicity $p_i$. 

In the simulation, each source samples items from a uniform distribution with $\hat{N}$ unique data items (i.e., a hypothetical population) without replacement; in effect, each item is assigned an index $i$ at random, and $p_i$ is just a relative frequency in the final merged sample over $n_w$ sources. On the other hand, we cannot randomly assign the index to the observed sample items. Ideally, the same item from $P_{S}$ and $Q_{\theta}$ would have the same index as they would in the population; however, it is not clear how the observed items should be ranked when there are missing unknown data items: should the unknown item have the largest, the third or the smallest value?


\begin{algorithm}\label{alg:mc_indexing}
\IncMargin{1em}
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Indm
\Input{a sample array of size $n$, $S$\\
        a set of indexes, $R$}
\Output{an indexed sample of size $n$, $S'$}
\Indp
\BlankLine
    $S' = sort(S)$\tcc*[r]{sort by value (desc)}
    $prev = max$\tcc*[r]{default value, max}
    \BlankLine
    \For{$i = 0$ \KwTo $n$}{
        $cur = S'[i]$\;
        \If{$prev > cur$}{
            \lIf{$empty(R)$}{$r=r+1$}
            \lElse(\tcc*[f]{pop min from $R$}){$r = popMin(R)$}
            $prev = cur$\;
        }
        $S'[i].index(r)$\tcc*[r]{assign index $r$}
    }
    \BlankLine
    return $S'$\;
    \caption{Sample indexing}
\end{algorithm}
\DecMargin{1em}

To handle the subtlety, we use the simulated indexes as in Algorithm~\ref{alg:mc_indexing}; the largest observed item is indexed with the smallest simulated index and so on. If the simulated index set is exhausted before indexing all observed items, then we increment the last used index by 1 and use it to index a remaining unique data item. If the simulated sample distribution is close to the observed sample distribution, then this indexing would result in smaller KL-divergence.

\subsubsection{Monte-Carlo Method Per Bucket}
The Monte-Carlo method in Algorithm~\ref{alg:mc_method} assumes a uniform sampling distribution for simulating $\hat{C}$ different data items. The true sampling distribution can take various forms and $p_i$ may be correlated to the value. Hence, the uniform sampling distribution is not the ...


